A Data Augmented Approach to Transfer Learning for Covid-19 Detection

Covid-19 detection at an early stage can aid in an effective treatment and isolation plan to prevent its spread. Recently, transfer learning has been used for Covid-19 detection using X-ray, ultrasound, and CT scans. One of the major limitations inherent to these proposed methods is limited labeled dataset size that affects the reliability of Covid-19 diagnosis and disease progression. In this work, we demonstrate that how we can augment limited X-ray images data by using Contrast limited adaptive histogram equalization (CLAHE) to train the last layer of the pre-trained deep learning models to mitigate the bias of transfer learning for Covid-19 detection. We transfer learned various pre-trained deep learning models including AlexNet, ZFNet, VGG-16, ResNet-18, and GoogLeNet, and fine-tune the last layer by using CLAHE-augmented dataset. The experiment results reveal that the CLAHE-based augmentation to various pre-trained deep learning models significantly improves the model efficiency. The pre-trained VCG-16 model with CLAHEbased augmented images achieves a sensitivity of 95% using 15 epochs. AlexNet works show good sensitivity when trained on non-augmented data. Other models demonstrate a value of less than 60% when trained on non-augmented data. Our results reveal that the sample bias can negatively impact the performance of transfer learning which is significantly improved by using CLAHE-based augmentation.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> asc.tex <==


\begin{thebibliography}{1}
\bibitem{tang1901}
Jie Tang, Shaoshan Liu, Bo Yu, Weisong Shi,PI-Edge, "A Low-Power Edge Computing System for Real-Time Autonomous Driving Services," preprint, 	arXiv:1901.04978v1.

\bibitem{kim2019}
S. Kim, D.-Y. Kim, J. -H. Park, "Traffic management in the mobile edge cloud to improve the quality of experience of mobile video," Comput. Commun. 2018, 118, pp. 40–49. 


\bibitem{yang18}
P. Yang, N. Zhang, S. Zhang, L. Yu, J. Zhang, and X. Shen, “Content Popularity Prediction Towards Location-Aware Mobile Edge Caching,” arXiv preprint arXiv:1809.00232, Sep. 2018.

\bibitem{sarkar18}
S. Sarkar, S. Chatterjee, and S. Misra, “Assessment of the Suitability of Fog Computing in the Context of Internet of Things,” IEEE Trans. Cloud Comput., 2018, 6(1), pp. 46-59.


\bibitem{zzhang18}
S. Zhang, P. He, K. Suto, P. Yang, L. Zhao, and X. Shen, “Cooperative edge caching in user-centric clustered mobile networks,” IEEE Trans. Mobile Comput., 2018, 17(8), pp. 1791-1805.

\bibitem{Nae11}
V. Nae, A. Iosup, and R. Prodan, “Dynamic resource provisioning
in massively multiplayer online games,” IEEE Trans. Parallel Distrib. Syst., 2011, 22(3), pp. 380-395.


\bibitem{Mohammadi18}
M. Mohammadi, A. Al-Fuqaha, S. Sorour, M. Guizani, "Deep learning for IoT big data and streaming analytics: A survey," IEEE Commun. Surv. Tutor. 2018, 20, pp. 2923–2960. 

\bibitem{Mahdavinejad18}
M.S. Mahdavinejad, M. Rezvan, M. Barekatain,P. Adibi, P. Barnaghi, A.P. Sheth, "Machine learning for internet of things data analysis: A survey," Digit. Commun. Netw. 2018, 4, pp. 161–175. 


\bibitem{Teerapittayanon17}
S. Teerapittayanon, B. McDanel, and H. T. Kung, “Distributed deep neural networks over the cloud, the edge and end devices,” in the 37th IEEE International Conference on Distributed Computing Systems, 2017.

\bibitem{li17}
S. Li, Q. Yu, M. A. Maddah-Ali, and A. S. Avestimehr, “A scalable framework for wireless distributed computing,” IEEE/ACM Transactions on Networking, 2017, 25(5), pp. 2643–2654.

\bibitem{park17}
E. Park, J. Ahn, S. Yoo, "Weighted-entropy-based quantization for deep neural networks," in CVPR '17, USA, 2017. 

\bibitem{hhan15}
S. Han, J. Pool, J. Tran, W.J. Dally, "Learning both weights and connections for efficient neural networks," in NIPS'15,Canada,2015, pp.7–12.

\bibitem{verhelst17}
M. Verhelst, B. Moons, "Embedded deep neural network processing: Algorithmic and processor techniques bring deep learning to IoT and edge devices," IEEE Solid-State Circuits Mag. 2017, 9, pp. 55–65.

\bibitem{lane16}
N.D. Lane, S. Bhattacharya, P. Georgiev,C. Forlivesi, L. Jiao, L. Qendro, F. Kawsar, "DeepX: A software accelerator for low-power deep learning inference on mobile devices," in IPSN'16, 2016, Austria, pp. 11-14.

\bibitem{lki18}
H. Li, K. Ota, M. Dong, "Learning IoT in edge: Deep learning for the internet of things with edge computing," IEEE Netw. 2018, 32, pp. 96–101. 

\bibitem{Konecn16}
J. Konecn y, H. B. McMahan, F. X. Yu, P. Richt arik, A. T. Suresh, and D. Bacon, “Federated learning: Strategies for improving communication efficiency,” arXiv preprint arXiv:1610.05492, 2016.

\bibitem{Scarsell09}
F. Scarselli, M. Gori, A. C. Tsoi, M. Hagenbuchner, and G. Monfardini, “The graph neural network model,” IEEE Trans. Neural Netw., 2009, 20(1), pp. 61–80.

\bibitem{branchy16}
S. Teerapittayanon, B. McDanel, H. Kung, "Branchynet: Fast inference via early exiting from deep neural networks", International Conference on Pattern Recognition, 2016.

\bibitem{Khelifi18}
H. Khelifi, S. Luo, B. Nour, A. Sellami, H. Moungla,S. H. Ahmed, and M. Guizani, “Bringing deep learning at the edge of information-centric internet of things,” IEEE Commun. Lett., 2018, pp. 1–1.

\bibitem{Arjevani15}
Y. Arjevani and O. Shamir, “Communication complexity of distributed convex learning and optimization,” in Advances in neural information processing systems, 2015, pp. 1756–1764.

\bibitem{zhang12}
Y. Zhang, M. J. Wainwright, and J. C. Duchi, “Communication-efficient algorithms for statistical optimization,” in Advances in Neural Information Processing Systems, 2012, pp. 1502–1510.


\bibitem{ma17}
C. Ma, J. Konecn y, M. Jaggi, V. Smith, M. I. Jordan, P. Richt arik, and M. Takac, “Distributed optimization with arbitrary local solvers,” Optimization Methods and Software, 2017, 32(4), pp. 813–848.


\bibitem{hli18}
H. Li, K. Ota, K., M. Dong, "Learning IoT in edge: Deep learning for the internet of things with edge computing," IEEE Netw. 2018, 32, pp. 96–101.



\bibitem{chen18}
X. Chen X, H. Zhang, C. Wu, S. Mao, Y. Ji, M. Bennis, "Performance optimization in mobile-edge computing via deep reinforcement learning," 2018, arXiv:1804.00514.
\bibitem{min17}
M. Min, D. Xu, L. Xiao, Y. Tang, D. Wu, "Learning-based computation offloading for IoT devices with energy harvesting," 2017, arXiv:1712.08768.

\bibitem{han15}
S. Han, J. Pool, J. Tran, W.J. Dally, "Learning both weights and connections for efficient neural networks," In Proceedings of the 28th International Conference on Neural Information Processing Systems (NIPS), 2015, Canada, pp. 7–12.


\bibitem{iandola16}
F.N. Iandola, S. Han, M.W. Moskewicz, K. Ashraf, W.J. Dally, K. Keutzer, "SqueezeNet: AlexNet-level accuracy with 50x fewer parameters and $<0.5$ MB model size. arXiv, 2016, arXiv:1602.07360v3.


\bibitem{ttang17}
J. Tang, D. Sun, S. Liu, J.L. Gaudiot, "Enable deep learning on IoT devices," Computer 2017, 50, pp. 92–96.

\bibitem{wang16}
Y. Wang, H. Li, X. Li, "Re-architecting the on-chip memory sub-system of machine-learning accelerator for embedded devices," In Proceedings of the 2016 IEEE/ACM International Conference on Computer-Aided Design (ICCAD), Austin, TX, USA, 2016, pp. 7-10.


\bibitem{du18}
L. Du, Y. Du, Y. Li, J. Su, Y.-C Kuan, C.-C. Liu, M.-C.F.A. Chang,  "Reconfigurable streaming deep convolutional neural network accelerator for internet of things," IEEE Trans. Circuits Syst. I Regul. Pap. 2018, 65, pp. 198–208.

\bibitem{che18}
X. Chen, H. Zhang et al., "Optimized Computation Offloading Performance in Virtual Edge Computing Systems via Deep Reinforcement Learning," arXiv:1805.06146, Nov. 2018.


\bibitem{howard17}
A. G. Howard, M. Zhu, B. Chen, D. Kalenichenko, W. Wang, T. Weyand, M. Andreetto, and H. Adam, “MobileNets: Efficient convolutional neural networks for mobile vision applications,” arXiv preprint
arXiv:1704.04861, 2017.


\bibitem{zhang17}
X. Zhang, X. Zhou, M. Lin, and J. Sun, “ShuffleNet: An extremely efficient convolutional neural network for mobile devices,” arXiv preprint arXiv:1707.01083, 2017.

\bibitem{mao17}
J. Mao, X. Chen, K. W. Nixon, C. Krieger, and Y. Chen, “MoDNN: Local distributed mobile computing system for deep neural network,”in Design, Automation Test in Europe Conference Exhibition (DATE),
2017.


\bibitem{li16}
Li, Dawei, et al. ”DeepCham: Collaborative Edge-Mediated Adaptive Deep Learning for Mobile Object Recognition,” Edge Computing (SEC), IEEE/ACM Symposium on. IEEE, 2016.

\bibitem{teera17}
S. Teerapittayanon, B. McDanel, H.T. Kung, "Distributed deep neural networks over the cloud, the edge and end devices," In IEEE International Conference on Distributed Computing Systems (ICDCS),2017, pp. 328–339.

\bibitem{Bhattacharya16}
S. Bhattacharya and N. D. Lane, “Sparsification and Separation of Deep Learning Layers for Constrained Resource Inference on Wearables,” In the 14th ACM Conf. Embedded Network Sensor Systems CD-ROM, ser. SenSys ‘16, 2016, pp. 176–89.


\bibitem{Alsheikh2016}
M. A. Alsheikh et al., “Mobile Big Data Analytics Using Deep Learning and Apache Spark,” IEEE Network, 2016, 30(3),pp. 22–29.


\bibitem{Liu17}
C. Liu et al., “A New Deep Learning-Based Food Recognition System for Dietary Assessment on an Edge Computing Service Infrastructure,” IEEE Trans. Services Computing. DOI: 10.1109/TSC.2017.2662008.

\bibitem{zhang18}
P. Zhang, M. Zhou, and G. Fortino, “Security and trust issues in fog computing: A survey,” Future Generation Computer Systems, 2018, 88,pp. 16–27.

\bibitem{jong18}
M. F. A. Jong Hwan Ko, Taesik Na and S. Mukhopadhyay, “Edge-host partitioning of deep neural networks with feature space encoding for resource-constrained internet-of-things platforms,” https://arxiv.org/pdf/1802.03835.pdf, 2018, arXiv Preprint.

\bibitem{Fwhilemi19}
F. Wilhelmi, S. Barrachina-Munoz, B. Bellalta, C. Cano, A. Jonsson, and ˜G. Neu, “Potential and pitfalls of multi-armed bandits for decentralized spatial reuse in {WLANs},” Journal of Network and Computer Applications, 2019, 127, pp. 26–42.

\bibitem{sergio18}
S ergio Barrachina-Munoz, Francesc Wilhelmi, Ioannis Selinis, and ˜
Boris Bellalta. Komondor: a Wireless Network Simulator for Next Generation High-Density WLANs. arXiv preprint arXiv:1811.12397,2018.

\bibitem{Yurii13}
Yurii Nesterov, "Introductory lectures on convex optimization: A basic course", Springer Science \& Business Media, 87, 2013.

\bibitem{boris64}
Boris T Polyak, "Some methods of speeding up the convergence of iteration methods," USSR Computational Mathematics and Mathematical Physics, 4(5):1–17, 1964.


\bibitem{esgd17}
Xinghao Pan Jianmin Chen Rajat Monga Samy Bengio and Rafal Jozefowicz. “Revisiting distributed synchronous {SGD}”, in: arXiv preprint:1702.05800, 2017. 

\bibitem{llin17}
Yujun Lin, Song Han, Huizi Mao, Yu Wang, and William J. Dally. “Deep Gradient Compression: Reducing the Communication Bandwidth for Distributed
Training”, In: arXiv:1712.01887, 2018.


\bibitem{Vaswani17}
A. Vaswani, N. Shazeer, N. Parmar, J. Uszkoreit, L. Jones, A. N. Gomez, Ł. Kaiser, and I. Polosukhin, "Attention is all you need," In Advances in Neural Information Processing Systems, 2017,pp. 6000–6010.









\end{thebibliography}

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{henna}}]{Shagufta Henna} is an assistant lecturer with the Letterkenny Institute of Technology Co. Donegal, Ireland. Recently she has been a post-doctoral researcher with the telecommunication software and systems group, Waterford institute of technology, Waterford, Ireland. She received her doctoral degree in Computer Science from the University of Leicester, UK in 2013. She is an Associate Editor for IEEE Access,EURASIP Journal on Wireless Communications and Networking, IEEE Future Directions, and Human-centric Computing and Information Sciences, Springer. Her current research
interests include edge computing, 5G and beyond, intent-based networking, distributed stochastic gradient, AI-driven network optimization.
\end{IEEEbiography}
% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Ad}}]{Alan Davy}
received the B.Sc. (with Hons.) degree in applied computing and the Ph.D. degree from
the Waterford Institute of Technology, Waterford, Ireland, in 2002 and 2008, respectively. Since 2002,
he has been with the Telecommunications Software and Systems Group, originally as a student and then,
since 2008, as a Post-Doctoral Researcher. He was a recipient of the Marie Curie International
Mobility Fellowship in 2010, which brought him to work at the Universitat Politecnica de Catalunya for two years. He is currently Head of Department of Computer Science, Waterford institute of technology, Waterford, Ireland. His current research interests include Virtualised Telecom Networks, Fog and Cloud Computing, Molecular Communications and TeraHertz Communication.
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

%\begin{IEEEbiographynophoto}{Jane Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks
\end{document}



